Implementing OpenMP for Zig to enable its use in HPC context

This extended abstract explores supporting OpenMP in the Zig programming language. Whilst, C and Fortran are currently the main languages used to implement HPC applications, Zig provides a similar level of performance complimented with several modern language features, such as enforcing memory safety. However, Zig lacks support for OpenMP which is the de facto threaded programming technology. Leveraging Zig's LLVM compiler tooling, we have added partial support for OpenMP to the Zig compiler and demonstrated that the performance attained by using Zig with OpenMP is comparable to, and in come cases exceeds, that of conventional HPC languages. Consequently we demonstrate that Zig is a viable and important programming technology to use for HPC, and this work paves the way for more HPC features to be added to Zig, ultimately providing HPC developers with the option of using a safer, more modern language for creating high performance applications.

==> latexmk <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -i dvipdfmx-unsafe.cfg -o %D %O %S";

# Workaround to allow pstricks transparency (https://github.com/overleaf/issues/issues/3449)
$dvipdf = "dvipdf -dNOSAFER -dALLOWPSTRANSPARENCY %O %S %D";

###############################
# Post processing of pdf file #
###############################

$compiling_cmd = "internal overleaf_pre_process %T %D";
$success_cmd = "internal overleaf_post_process %T %D";
$failure_cmd = $success_cmd;

# equivalent to -gt option. Used to prevent latexmk from skipping recompilation
# of output.log and output.pdf
$go_mode = 3;

# equivalent to -bibtex option. Run bibtex unconditionally when bbl files are
# out of date.
$bibtex_use = 2;

my $ORIG_PDF_AGE;

sub overleaf_pre_process {
    my $source_file = $_[0];
    my $output_file = $_[1];

    # get age of existing pdf if present
    $ORIG_PDF_AGE = -M $output_file
}

sub overleaf_post_process {
    my $source_file = $_[0];
    my $output_file = $_[1];
    my $source_without_ext = $source_file =~ s/\.tex$//r;
    my $output_without_ext = $output_file =~ s/\.pdf$//r;

    # Look for a knitr concordance file
    my $concordance_file = "${source_without_ext}-concordance.tex";
    if (-e $concordance_file) {
        print "Patching synctex file for knitr...\n";
        system("patchSynctex.R", $source_without_ext, $output_without_ext);
    }

    # Return early if pdf file doesn't exist or wasn't updated
    my $NEW_PDF_AGE = -M $output_file;
    return if !defined($NEW_PDF_AGE);
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE;

    # Figure out where qpdf is
    $qpdf //= "/usr/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf;
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});

    # Run qpdf
    my $optimised_file = "${output_file}.opt";
    system($qpdf, split(' ', $qpdf_opts), $output_file, $optimised_file);
    $qpdf_exit_code = ($? >> 8);
    print "qpdf exit code=$qpdf_exit_code\n";

    # Replace the output file if qpdf was successful
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($qpdf_exit_code == 0 || $qpdf_exit_code == 3);
    print "Renaming optimised file to $output_file\n";
    rename($optimised_file, $output_file);

    print "Extracting xref table for $output_file\n";
    my $xref_file = "${output_file}xref";
    system("$qpdf --show-xref ${output_file} > ${xref_file}");
    $qpdf_xref_exit_code = ($? >> 8);
    print "qpdf --show-xref exit code=$qpdf_xref_exit_code\n";
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
add_cus_dep( 'Rtex', 'tex', 0, 'do_knitr');
add_cus_dep( 'Rnw', 'tex', 0, 'do_knitr');
sub do_knitr {
    Run_subst(qq{Rscript -e '
        library("knitr");
        opts_knit\$set(concordance=T);
        knitr::knit(%S, output=%D);
        '}
    );
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############

sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/local/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}

